Rank-decreasing transductions

We propose to study transformations on graphs, and more generally structures, by looking at how the cut-rank (as introduced by Oum) of subsets is affected when going from the input structure to the output structure. We consider transformations in which the underlying sets are the same for both the input and output, and so the cut-ranks of subsets can be easily compared. The purpose of this paper is to give a characterisation of logically defined transductions that is expressed in purely structural terms, without referring to logic: transformations which decrease the cut-rank, in the asymptotic sense, are exactly those that can be defined in monadic second-order logic. This characterisation assumes that the transduction has inputs of bounded treewidth; we also show that the characterisation fails in the absence of any assumptions.

==> almost-commutative.tex <==
\section{Almost commutative semigroups}

For a semigroup $S$, define the \emph{syntactic congruence on $S^k$} as follows. (When $k=1$ then this is the usual syntactic congruence.) Two tuples 
\begin{align*}
(a_1,\ldots,a_k), (b_1,\ldots,b_k) \in S^k
\end{align*}
are considered equivalent if for every 
\begin{align*}
(c_0,\ldots,c_k) \in S^{k+1} + \varepsilon
\end{align*}
we have 
\begin{align*}
c_0a_1c_1a_2c_2 \cdots a_kc_k  =  c_0b_1c_1b_2c_2 \cdots b_kc_k.
\end{align*}
We are interested in the number of equivalence classes of this relation, as a function of $k$. If the semigroup is commutative, then the number of equivalence classes is bounded, since the equivalence class of $(a_1,\ldots,a_k)$ is simply determined by its product. The following theorem shows that commutativity is roughly the only condition. In a commutative semigroup, the product of a sequence of semigroup elements depends only on the underlying multiset. In the following theorem, we use a relaxation of this condition: we are allowed to look at a prefix and suffix of constant size, but otherwise 

\begin{theorem}\label{thm:semicommutative}
    For a finite semigroup $S$, the following conditions are equivalent: 
    \begin{enumerate}
        \item \label{semicommutative:equation} The semigroup satisfies the equation
        \begin{align*}
        exyf = eyxf \qquad \text{for every $e,x,y,f \in S$ with $e,f$ idempotent}.
        \end{align*}
        \item \label{semicommutative:logical} There is some $k \in \set{0,1,\ldots}$ such that for every $w \in S^+$, the value of the semigroup product of $w$ depends only on: (a) the prefix consiting of the first  $k$ letters; (b) the suffix consisting of the last $k$ letters; (c) the multiset of letters.
        \item \label{semicommutative:congruence} There is some $\ell$ such that for every $k$, there are at most $\ell$ equivalence classes of syntactic congruence on $S^k$. 

    \end{enumerate}
\end{theorem}
\begin{proof}
    

    Let $\omega \in \set{1,2,\ldots}$ be a number such that for every element $s \in S$ in the semigroup, its power $s^\omega$ is an idempotent. Such a number is guaranteed to exist in every finite semigroup. 

    \begin{claim}\label{claim:idempotents-cyclic}
        Assume \ref{semicommutative:congruence}. Then for every idempotents $e,f$, we have 
        \begin{align*}
        ef = (ef)^{\omega+1}.
        \end{align*}
    \end{claim}
    \begin{proof}
        An equivalent statement of the claim is that for every idempotents $e,f$, the subsemigroup generated by the element $ef$ is a cyclic group.  We will prove the contrapositive of the claim: a violation of the identity will lead to a violation of~\ref{semicommutative:congruence}. Consider some idempotents $e,f$ that are a violation of the identity, i.e.~
        \begin{align*}
        ef \neq (ef)^{\omega +1}.
        \end{align*}
        For numbers $a,b,c \in \set{1,2,\ldots}$  consider  two sequences of semigroup elements 
        \begin{align*}
        e^{a+b} f^{c} 
        \quad 
        e^{a} f^{b+c}.
        \end{align*}
        These sequences  have length $a+b+c$ and they are  described in the following picture:
        \mypic{1}
        We will use an environment to distinguish them as in the following picture:
        \mypic{2}
        Under this environment, the values of the upper and lower sequences are 
        \begin{align*}
            \myunderbrace{e^{2a-1} (ef)^{b+1} f^{2c} = (ef)^{b+1}}{upper sequence}
            \qquad 
            \myunderbrace{e^{2a+1}f^{2b+2c} = ef}{upper sequence}.
        \end{align*}
        If we assume that $b$ is a multiple of $\omega$, then the upper and lower sequence have different values in the specified environment, by choice of $e$ and $f$ as a violation of the identity. Therefore, we know that for every $a,b,c$ with $b$ being a multiple of $\omega$, the two corresponding sequences can be distinguished in some environment. This means that for every $n \in \set{1,2,\ldots}$, all of the sequences 
        \begin{align*}
            \setbuild{ e^{i\omega} f^{n-i\omega}}{ $0 < i \omega < n$}
        \end{align*}
        are pairwise distinguishable by some environment. Since the number of such sequences grows with $n$, we obtain a violation of condition~\ref{semicommutative:congruence}.
    \end{proof}
    
    \begin{claim}\label{claim:e-semigroup}
        Assume \ref{semicommutative:congruence}. Then for every idempotents $e,f$, we have 
        \begin{align*}
        ef = efef
        \end{align*}
    \end{claim}
    \begin{proof}
        In other words, the claim says that the product of two idempotents is also an idempotent; in other words  the idempotents form a subsemigroup. By Claim~\ref{claim:idempotents-cyclic}  we know the subsemigroup generated by $ef$ is a cyclic group of some order $n$. We need to show that the order of this group is $n=1$. 
    \end{proof}

    \begin{claim}\label{claim:exef}
        Assume \ref{semicommutative:congruence}. Then for every $e,f,x$ with $e,f$ idempotent  we have 
        \begin{align*}
        exf = exef.
        \end{align*}
    \end{claim}
    \begin{proof}
        We use a similar proof as for Claim~\ref{claim:idempotents-cyclic}, but we also Claim~\ref{claim:e-semigroup}. As in Claim~\ref{claim:idempotents-cyclic}, we prove the contrapositive: a violation of the identity $exf=exef$ would lead to a violation of~\ref{semicommutative:congruence}. Let $e,x,f$ be elements that lead to such a violation. 
         We use the same sequences as in the proof of Claim~\ref{claim:idempotents-cyclic}, but a different environment to distinguish them. This environment is depicted in the following picture: 
         \mypic{3}
         Combining the upper and lower sequences with the environment gives us the values
         \begin{align*}
            \myunderbrace{ex(ef)^b}{upper sequence}
            \qquad  \qquad 
            \myunderbrace{exf}{lower sequence}.
        \end{align*}
        Thanks to Clam~\ref{claim:e-semigroup}, the upper value corresponding to the upper sequence is equal to $exef$, and therefore the upper and lower sequences can be distinguished by the environment.
    \end{proof}

    We now prove the final identity 
    \begin{align*}
    exyf=eyxf.
    \end{align*}
    As previously, we use a violation of this identity to prove a violation of~\ref{semicommutative:congruence}. Suppose that elements $e,f,x,y$ witness a violation of this identity. Consider the following two sequences and a distinguishing environment:
    \mypic{4}
    The values of these two sequences in the environment are equal to, respectively:
    \begin{align*}
        \myunderbrace{ey(ef)^bxf}{upper sequence}
        \qquad  \qquad 
        \myunderbrace{exyf}{lower sequence}.
    \end{align*}
    For the upper sequence, we have 
    \begin{align*}
    ey(ef)^{b}xf 
    \stackrel{\text{Claim~\ref{claim:e-semigroup}}} = 
    eyefxf 
    \stackrel{\text{Claim~\ref{claim:exef}}} = 
    eyfxf 
    \stackrel{\text{Claim~\ref{claim:exef}}} = 
    eyxf 
    \end{align*}


    \begin{claim}Condition \ref{semicommutative:congruence} implies the following identities, for $x,y,e,f \in S$ with $e$ and $f$ idempotent: 
    \begin{eqnarray}
        ef & = efef \label{eq:ef}\\
    exf & = exef  \label{eq:exf}\\ 
    exye & = eyxe \label{eq:exye} 
    \end{eqnarray}
    \end{claim} 
    Before proving the claim, we use it to show the  Condition~\ref{semicommutative:congruence} in the theorem implies Condition~\ref{semicommutative:equation}. Thanks to the claim, we can use the identities~\eqref{eq:exf} and~\eqref{eq:exye}. (The first identity~\eqref{eq:ef} is used inside the proof of the claim.) Therefore, we have 
    \begin{align*}
    exyf   \stackrel  {\text{\eqref{eq:exf}}} = 
    exyef \stackrel  {\text{\eqref{eq:exye}}} = 
    eyxef \stackrel  {\text{\eqref{eq:exf}}} = 
    eyxf 
    \end{align*}
    which proves Condition~\ref{semicommutative:equation}. It remains to prove the claim. 
    \begin{proof}
        We first prove the identity 
        \begin{align}\label{eq:efef}
        ef = efef
        \end{align}
        We prove the contrapositive:  a violation of either of the two identities would lead to a violation of~\ref{semicommutative:congruence}. Consider first a violation of the first identity. We will show that for every $k$, the elements 
        \begin{align*}
        w_{ij} = [\myunderbrace{e,\ldots,e}{$i$ times}, \myunderbrace{f,\ldots,f}{$j$ times}]
        \end{align*}
        We will show that if there is a violation of this identity, then 
        \begin{align*}
        \setbuild{ w_{i\omega, (n-i)\omega}}{$1 < i < n$}
        \end{align*}
        
        This proves that there is some $\ell$ such that 
        \begin{align*}
        ef = (ef)^\ell.
        \end{align*}
        In other words, the element $ef$ generates a subsemigroup that is isomorphic to cyclic group. We now show that $\ell = 1$, i.e.~the cyclic group is trivial. Consider two 
        \begin{align*}
            w_{ij}
        \end{align*}
    \end{proof}
    We show that~\ref{semicommutative:congruence} implies 
    \begin{align*}
    exf = exef
    \end{align*}
\end{proof}



% \bibliographystyle{plain}
% \bibliography{bib}

\begin{lemma}
    For an linear order and $\ell \in \set{1,2,\ldots}$, consider the property 
    \begin{quotation}
        $R_\ell(X) = $the set $X$ is a union of $\ell$ intervals.
    \end{quotation}
    There is an \mso formula that defines $R_1(X)$ in terms of $R_\ell(X)$. 
\end{lemma}


The hyperedges in a  hypergraph with vertices $V$ are described by a function of type  
\begin{align*}
2^V \to 2.
\end{align*}
We can consider a mild generalisation, the function has  type 
\begin{align*}
k^V \to k
\end{align*}
for some $k \in \set{1,2,\ldots}$. Such a generalisation will be called a \emph{$l$-valued hypergraph}. A $k$-valued hypergraph can be seen as a model. In this model, the universe is the set of vertices. The hyperedge information is modelled by $k$ relations 
\begin{align*}
R_1,\ldots,R_k \quad \text{of type } \myunderbrace{\text{(set, ..., set)}}{$k$ times}.
\end{align*}
The $i$-th relation inputs sets $X_1,\ldots,X_k$ and says ``yes'' if the sets form a parition of the universe, and the correponding colouring of elemenets gives value $i$ in the hypergraph. 


Suppose that $S$ is a semigroup. For a number $n \in \set{1,2,\ldots}$ we can define an $S$-valued hypergraph as follows.  The vertices are  $\set{1,\ldots,n}$. The value of a hyperedge, which can be seen as a word 
\begin{align*}
[s_1,\ldots,s_n] \in S^n
\end{align*}
is simply the product of the word in the semigroup. 

\begin{lemma}
    For every finite semigroup $S$, the class 
    \begin{align*}
    \setbuild{S(n)}{$n \in \set{1,2,\ldots}$}
    \end{align*}
    has definable tree decompositions.
\end{lemma}
\begin{proof}
    We consider the two cases for the semigroup $S$ that can arise by applying Theorem~\ref{thm:semicommutative}. 

    \begin{itemize}
        \item \emph{Semi-commutative.} Suppose first that $S$ is semicommutative. Let $k$ be the number in the definition of semicommutative. The \mso transduction inputs a hypergraph $S(n)$, and nondeterministically distinguishes $2k$ elements. The idea is that these are the lefmost $k$ elements and the rightmost $k$ elements. 
        To know the value of a hyperedge 
        \begin{align*}
        \lambda \in S^n
        \end{align*}
        in $S(n)$, we need to know (a) the colours under $\lambda$ of the first $k$ vertices in $\set{1,\ldots,n}$, (b) the colours under $\lambda$ of the last $k$ vertices in $\set{1,\ldots,n}$, and (c) the multiset of colours of all vertices.  Furthermore, in item (c) the multiset needs only to be known modulo some recognizabile property of multisets, which boils down to computing the size of a multiset modulo some fixed number, and up to some fixed threshold. All of this can be defined in \mso, assuming that we know which of elements are the $k$ leftmost and which ones are the $k$ rightmost. 
        \item \emph{Not semi-commutative.} Suppose that 
    \end{itemize}
\end{proof}

==> approx.tex <==
\section{Improving a transduction to one that is complexity preserving}

In this section, we show that if a transduction 

\begin{theorem}
    Let $\Cc$ be a class of structures of bounded linear width. Then there is a surjective complexity preserving tree-to-$\Cc$ transduction.
\end{theorem}
\subsection{Tree decompositions}

Define a \emph{tree decomposition} for a structure $\structa$ to be a tree order on it 

\begin{definition}[Linear decompositions and width]
    Define a \emph{linear decomposition} for a structure to be a linear order on its universe. The \emph{width} of such a decomposition is defined to be the maximal logical complexity of downsets. A class of structures has \emph{bounded linear width} if there is some $k$ such that for every structure in the class, there is a linear decomposition of width at most $k$.
\end{definition}

There is a related, and arguably more fundamental, notion of tree decomosition. In a tree decomosition, instead of a linear order, we use a binary tree whose set of leaves is the universe of the structure, and the complexity is measured for subtrees, i.e.~sets of leaves that arise by taking all descendant of some node in the tree. In this paper, we do not deal with tree decompositions. 

We believe that the logical view on tree decompositions is useful. For example, it is clear that grids do not have bounded width, even if we allow tree decompositions. This is because in a tree decomposition of a large grid there will necessarily be a  subtree with many vertices from the grid, and according to Example~\ref{ex:grid-complexity}, the size of a subset in a grid is asymptotically equivalent to its logical complexity. (To be fair, this is essentially the same reasoning as the classical argument for why grids have unbounded width, only .)


In this section, we study classes of structures that arise as images of complexity preserving transduction from trees of bounded height.




\subsection{Hypergraphs}


\begin{theorem}[Not yet proved]\label{thm:all-is-good}
 If there is a tree-to-$\Cc$ transduction that is definable, surjective and has inputs of bounded height, then there is a tree-to-$\Cc$ transduction that has all the above properties, and is furthermore complexity preserving. 
\end{theorem}

In order to save space, we give a (not particularly imaginative) name to transductions as in the conclusion of the above theorem. 
\begin{definition}\label{def:good}
 We say that a transduction is \emph{good} if its inputs are trees of bounded height, and it is complexity preserving. 
\end{definition}
Not that by Theorem~\ref{thm:complexity-decreasing}, good transductions are automatically definable. Using the terminology from Definition~\ref{def:good}, the statement of Theorem~\ref{thm:all-is-good} becomes: for every definable tree-to-$\Cc$ transduction which has inputs of bounded height, there is a good transduction whose set of outputs is at least as big. 
The purpose of this section is to prove Theorem~\ref{thm:all-is-good}.
The general strategy behind the proof is to show that good transductions have certain closure properties and, by Simon's Factorisation Forest Theorem, these closure properties are enough to cover all images of definable tree-to-$\Cc$ transductions. The first obvious property is that good transductions are closed under (not necessarily disjoint) union and taking subsets.
\begin{lemma}
 \label{lem:union-subset} Good transductions are closed under finite unions and subsets.
\end{lemma}

The remaining two closure properties are less obvious (with the last one being still open at the time of writing). 

\paragraph*{Hypergraphs.}
For the remaining properties, it will be more convenient to use hypergraph terminology, as described below. 

\begin{definition}[Hypergraphs]\label{def:hypergraphs} A \emph{hypergraphs} consists of: 
    \begin{enumerate}
        \item a set $V$ of vertices;
        \item a set $A$ of output colours;
        \item an edge function of type $\powerset V \to A$.
    \end{enumerate} 
\end{definition}
We use the name $A$-hypergraphs for hypergraphs with colours $A$. The usual notion of hypergraph is when there are two output colours ``yes'' and ``no'', but more output colours will be useful in this paper. A hypergraph is called \emph{surjective} if its edge function is surjective, i.e.~every output colour is achieved by some subset of the vertices. 

A structure over a vocabulary $\Sigma$ can be seen as a hypergraph, where the set of output colours is $\powerset \Sigma$. In this hypergraph, every subset is mapped to the set of relation names that select it. Conversely, a hypergraph with output colours $A$ can be seen as a structure over a vocabulary that has one relation per element $a \in A$; this relation selects the subsets that are mapped to $a$ by the edge function. It is this representation that we use when talking about transductions or logic for hypergraphs.

\subsection{Kronecker product of good transductions}
\label{sec:Kronecker-product-of-good-transductions}
We now show that good transductions are closed under a certain form of pairing. When pairing structures use an operation called Kronecker product.
Recall the notion of matrix from Section~\ref{sec:measure}. This is simply a binary operation, which can be illustrated in the style of string diagrams as follows: 
\mypic{12}
A matrix can be used to combine two graphs. 

\begin{definition}[Kronecker product of hypergraphs] Let $G$ and $H$ be hypergraphs, and let 
    \begin{align*}
    M : \text{(output colours of $G$)} \times \text{(output colours of $H$)} \to A
    \end{align*}
    be a matrix. The \emph{Kronecker product} of $G$ and $H$ along $M$, denoted by $G \graphproduct M H$, is the following hypergraph. The set of vertices is the disjoint union of the vertices in $G$ and $H$. The set of output colours is $A$. The edge function is defined by applying $G$ and $H$ to the respective parts, and combining the result using the matrix $M$.
\end{definition}

The goal of this section is to show that good transductions can be combined using Kronecker product on the output hypergraphs, and tree pairing on the input trees. To achieve this, however, we will need to make an assumption on the matrix used in the Kronecker product: the matrix must be irredundant.

\begin{definition}[Irredundant matrix]
    A matrix is called \emph{irredundant} if it every two columns can be distinguished by some row, and every two rows can be distinguished by some column.
\end{definition}
  
%  
We now state the first lemma about combining good transductions. In the lemma, a graph is called \emph{surjective} if every output colour is achieved by some subset of vertices.
\begin{lemma}\label{lem:binary-good}
 Let $A_1,A_2,A$ be finite sets, let 
 \begin{align*}
 M : A_1 \times A_2 \to A,
 \end{align*}
 be an irredundant matrix, and let $\Cc_1,\Cc_2$ be images of good transductions, such that $\Cc_i$ is a class of surjective hypergraphs with output colours $A_i$. Then there is a good transduction with image 
 \begin{align*}
 \Cc_1 \graphproduct M \Cc_2 \eqdef \setbuild{G_1 \graphproduct M G_2}{$G_1 \in \Cc_1$ and $G_2 \in \Cc_2$}.
 \end{align*}
 \ 
\end{lemma}

The rest of Section~\ref{sec:Kronecker-product-of-good-transductions} is devoted to proving the above lemma. In the proof, we will view the irredundant matrix $M$ as an operation on not just graphs, but also on matrices. Suppose that we have two matrices $M_1$ and $M_2$, with $M_i$ having type 
\begin{align*}
M_i : X_i \times Y_i \to A_i
\end{align*}
Suppose also that we have some kind of aggregation mechanism for the two outputs, which itself is a matrix
\begin{align*}
M : A_1 \times A_2 \to A.
\end{align*}
Using this aggregation mechanism, we can combine the two matrices into a single one, which is also called their \emph{Kronecker product}, is denoted by 
\begin{align*}
 M_1 \graphproduct M M_2 : \underbrace{X_1 \times X_2}_{X} \times \underbrace{Y_1 \times Y_2}_{Y} \to A,
\end{align*}
and is defined by 
\begin{align*}
((x_1,x_2),(y_1,y_2)) \mapsto M(M_1(x_1,y_1),M_2(x_2,y_2)).
\end{align*}
The corresponding string diagram is 
\mypic{13}


 The main observation behind the proof is the following claim about matrices. 
 
 \begin{claim}\label{claim:matrix-irredundant-binary-product}
 Let $M : A_1 \times A_2 \to A$ be an irredundant matrix. Then
 \begin{align*}
 \boundeq{
 \text{rank of $M_1 \graphproduct M M_2$}
 }
 {M_1 \in \text{surjective $A_1$-matrices}\\
 M_2 \in \text{surjective $A_2$-matrices}}
 {
 \max_{i = 1,2}{\text{rank of $M_i$}}
 }
 \end{align*}
 \end{claim}
 \begin{proof} Consider a set of $\Xx$ of arguments $(M_1,M_2)$. We need to show that the left side of the equivalence in the statement of the claim is unbounded over $\Xx$ if and only if the right side is unbounded. 

 The straightforward implication is $\Rightarrow$, i.e.~if the left side is unbounded then the right side is unbounded. This is because the number of rows in the matrix $M_1 \graphproduct M M_2$ is at most the product (i.e.~multiplication) of the number of rows in the matrices $M_1$ and $M_2$. 
 
 The more interesting implication is $\Leftarrow$, i.e.~if the right side is unbounded then the left side is unbounded; in this implication we use the assumption that the matrix is irredundant. Suppose that the right side is unbounded. This means that there is some $i \in \set{1,2}$ such that the complexity of $M_i$ is unbounded. 
 By symmetry we can assume without loss of generality that $i=1$.
 Because the $A_2$-matrices are surjective, we know that every $a_2 \in A_2$ appears in the range of every matrix $M_2$. This means that for every $a_2 \in A_2$, and every $(M_1,M_2) \in \Xx$, 
 \begin{align}
 \label{eq:distinguishing-element-in-the-other-matrix}
 M_1 \graphproduct M a_2 \text{ is a submatrix of } M_1 \graphproduct M M_2.
 \end{align}

 Because the rank of the $M_1$ matrices is unbounded, we can use a Ramsey argument to prove that there are some elements $a_1 \neq a_1' \in A_1$ such that for every $n$, there is some matrix $M_1$ which has $n$ distinguished rows with the following property: if $x,x'$ are two distinguished rows, then there is some column $y$ such that $M_1(x,y)=a_1$ and $M_1(x',y)=a_1'$. Because $M$ is irredundant, we know that there is some $a_2 \in A_2$ such that 
 \begin{align*}
 M(a_1,a_2) \neq M(a_1',a_2).
 \end{align*}
 Combinig this with~\eqref{eq:distinguishing-element-in-the-other-matrix}, we see that the matrix $M_1 \graphproduct M M_2$ has at least $n$ distinct rows.
 \end{proof} 
 
 We will use the above claim to prove the lemma. 
 Let $\varphi_1,\varphi_2$ be the two transductions in the assumption of the lemma. We combine these two transductions in the obvious way, i.e.~it consists of input/output pairs of the form \begin{align*}
 \myunderbrace{(T_1,T_2)}{a pair of trees is viewed as a tree\\ where the root has two child subtrees $T_1$ and $T_2$} \mapsto G_1 \graphproduct M G_2
 \end{align*}
 such that $T_1 \stackrel {\varphi_1} \mapsto G_1$ and $T_2 \stackrel {\varphi_2} \mapsto G_2$. Let us argue that the transduction $\varphi$ defined this way is good.
 
 
 The first observation is that the complexity of a subset of nodes in a graph $G_1 \graphproduct M G_2$ is the maximum of the complexities in the two graphs:
 \begin{align*}
 \boundeq{
 \text{complexity of $U_1 \cup U_2$ in $G_1 \graphproduct M G_2$}
 }
 {G_1 \in \text{surjective $A_1$-graphs}\\
 G_2 \in \text{surjective $A_2$-graphs} \\
 U_1 \subseteq G_1\\
 U_2 \subseteq G_2}
 {
 \max_{i = 1,2}{\text{complexity of $U_i$ in $G_i$}}
 }
 \end{align*}
 The above equivalence is a direct corollary of Claim~\ref{claim:matrix-irredundant-binary-product}, by mapping each pair $(G_i,U_i)$ to the corresponding matrix $M_i$. A similar result holds for trees: 
 \begin{align*}
 \boundeq{
 \text{complexity of $U_1 \cup U_2$ in $(T_1,T_2)$}
 }
 {T_1,T_2 \in \trees \\ 
 U_1 \subseteq T_1\\
 U_2 \subseteq T_2}
 {
 \max_{i = 1,2}{\text{complexity of $U_i$ in $T_i$}}.
 }
 \end{align*}
 In fact, the result for trees is a corollary of the result for graphs, since a tree can be seen as a special case of a graph. Combining the two assymptotic equivalences above we get the lemma. 

\subsection{Kleene star}
In the previous lemma, we dealt with hypergraphs where the set of output colours has no structure. In the following lemma, the colours will have a semigroup structure. In such a case, the hyperegraphs themselves form a semigroup. If $\Cc$ is a class of $A$-hypergrtaphs, then we write $\subalgebra \Cc$ for the sub-semigroup generated by $\Cc$, in the semigroup of graphs that have output colours $A$. This notation is only meaningful when $A$ is a semigroup. 
\begin{lemma}\label{lem:idempotent-good}
 Let $A$ be a finite semigroup, which satisfies the following conditions: 
 \begin{enumerate}
 \item $A^2 = A$;
 \item for every $a \neq b \in A$ there exist $x,y \in A$ with $xay \neq xby$.
 \end{enumerate}
 If $\Cc$ is a class of surjective $A$-hypergraphs, and there is a good trasndcution with range $\Cc$, then there is also a good transduction with range $\subalgebra \Cc$. 
\end{lemma}

The above lemma is the heart of our construction. It will be proved in Section~\ref{sec:idempotent-good}.

\subsection{Proof of Theorem~\ref{thm:all-is-good}}
Using Factorisation forests.


==> assymptotic.tex <==
In this section we introduce some notation and examples that will be used later in the paper. 




==> definable-extensions.tex <==
\section{Definable extensions}
Define a \emph{relation} over a universe $V$, with $k$ element arguments and $\ell$ set arguments, to be a subset of 
\begin{align*}
R \subseteq V^k \times (\powerset V)^\ell.
\end{align*}
A \emph{structure} is defined to be a set, called the universe, together with a family of relations. For a structure $\structa$ and a relation $R$ on this structure, its \emph{\mso complexity} is defined to be the smallest number $k$ such that $R$ can be defined by a formula of \mso, with the same type as $R$, that is allowed to use set parameters, and which has quantifier rank at most $k$ and at most $k$ set parameters.

Consider two relational structures $\structa$ and $\structb$. We say that $\structb$ \emph{extends} $\structa$, which is written as $\structa \le \structb$,  if $\structb$ can be obtained from $\structa$ by adding some new relations. In particular, the two structures have the same underlying set. The \emph{\mso complexity} of an extension is the smallest $k$ such that each of the new relations in $\structb$ has \mso complexity at most $k$ in the original structure $\structa$. 

\subsection{Trees}
One special case of a structure that we use is trees, in the following sense. A tree is defined to be a hypergraph where: (a) the full set is a hyperedge; (b) every singleton is a hyperedge; and (c) every two hyperedges are either disjoint, or related by inclusion.

\begin{lemma} For every tree $(V,\Tt)$ and every family $\Rr \subseteq \Tt$, 
    \begin{align*}
    (V,\Tt) \stackrel 7 \le (V,\Tt,\Rr)
    \end{align*}
\end{lemma}







==> generator-matrix.tex <==
\section{Matrices with generators}
The purpose of this section is proving the following theorem. 

\begin{theorem}
   \label{thm:finitary-generator}
        Let $A$ be a semigroup with $A^2=A$. If $\Sigma \subseteq A$ is a subset that generates $A$, and the matrix $\multmat A \Sigma$ is finitary, then the semigroup $A$ is almost commutative. 
\end{theorem}
In particular, if the semigroup satisfies the assumptions of the above theorem, and furthermore every two elements can be distinguished in a nonempty environment, then the semigroup is commutative, and not only almost commutative. 

For the rest of this section we fix a semigroup $A$ with $A^2=A$. 
We begin with a lemma that will be our main interface to the assumption that the matrix $\multmat \Sigma A$ is finitary.  Nevertheless, in the lemmas below we try to identify which of the assumptions are used, so that the lemmas could possibly be used in other contexts. 

\begin{lemma}\label{lem:swallow-idempotents}
    Let $A$ be a semigroup with $A^2=A$. If $\Sigma \subseteq A$ is a subset that generates $A$, and the matrix $\multmat A \Sigma$ is finitary, then 
\begin{align}\label{eq:swallow-idempotents}
    ef = egf \qquad \text{for every idempotents $e,f,g \in A$ with $g$ generated by $\jdown e \cup \jdown f$}
\end{align}
\end{lemma}
\begin{proof}
    We begin with the following claim, which will also be used outside the present lemma. 
    \begin{claim}\label{claim:multmat-tool}
        Assume that $\multmat \Sigma A$ is finitary. 
        Let $a,b,e,f \in A$ be such that $e$ and $f$ are idempotents, and let $x,y$ be generators that appear in $e$ and $f$, respectively. Then 
        \begin{align*}
        e a(xb)^! f = ea(yb)^! f 
        \end{align*}
    \end{claim}
    \begin{proof}
        Consider a power of the matrix $\multmat \Sigma A$ that is divisible by $!$. Consider lines of this matrix in which some prefix of length divisible by $!$ uses the letter $x$, and the rest of the letters are $y$. Here is a picture of two such lines: 
        \mypic{11}
        There is a column of the matrix, such that the corresponding cells for both lines are the two sides of the equation in the statement of the lemma, as explained in the following picture:
        \mypic{10}
        Therefore, the two sides of the equation must be equal, since otherwise we could separate every pair of lines with some column. 
    \end{proof}

    
    Fix for the rest of this proof two idempotents $e$ and $f$. 
    
    \begin{claim}\label{claim:swap-two-letters}
        Let $x$ and $y$ be generators such that appear in $e$ and $f$ and respectively.  Then  
        \begin{align*}
        e(axb)^! f = e(ayb)^! f
        \qquad \text{for every $a,b \in A+\varepsilon$.}
        \end{align*}
    \end{claim}
    \begin{proof}
        A corollary of Claim~\ref{claim:multmat-tool}.
    \end{proof}
    Let $\approx$ be the equivalence relation on $A$ defined by 
    \begin{align*}
    x \approx y
    \quad \iff \quad 
    e(axb)!f = e(ayb)!f \quad \text{ for all $a,b \in A + \varepsilon$}.
    \end{align*}
    This equivalence relation depends on the choice of fixed idempotents $e$ and $f$. Claim~\ref{claim:swap-two-letters} shows that $x \approx y$ holds for every generators $x$ and $y$ that appears in $e$ and $f$, respectively. By transitivity, it follows that $x \approx y$ holds for every generators such that each one of them appears in either $e$ or $f$. It is not hard to see that $\approx$ is a congruence. Therefore, it follows that $x \approx y$ holds for every $x$ and $y$ that are generated by generators that appear in either $e$ or $f$, thus establishing the lemma. 
\end{proof}


We say that two elements $a, b \in A$ \emph{have a common prefix} if there exists some element that is a prefix (possibly a proper prefix) of both $a$ and $b$.  Symmetrically we talk about having a common suffix. In the following lemma, we only use the property~\eqref{eq:swallow-idempotents} that was proved in the previous lemma. 
\begin{lemma}\label{lem:common-prefix-suffix}
    Let $A$ be a semigroup thaty satisfies~\eqref{eq:swallow-idempotents}.
    Let $e$ and $f$ be idempotents that are in the same $\Jj$-class, and such that $e$ and $f$ have a common prefix, and also have a common suffix. Then $e=f$.
\end{lemma}
\begin{proof}
    We will show a slightly stronger claim. 
    \begin{claim}
        If $e$ and $f$ are idempotents in the same $\Jj$-class, and they have a common prefix, then they are prefix equivalent. 
    \end{claim}

    Before proving the claim, we show how it implies the lemma. By the claim, and a symmetric variant for suffixes, it follows that if $e$ and $f$ satisfy the assumptions of the lemma, then they are both prefix and suffix equivalent. In other words, they are  in the same $\Hh$-class.     Since every $\Hh$-class contains exactly one idempotent, they must be equal. It remains to prove the claim. 
    
    \begin{proof}
        Consider a common prefix 
        \begin{align*}
        e = xa \qquad f = xb
        \end{align*}
        Like for any element, there is an idempotent infix of $x$, i.e.~it can be decomposed as 
        \begin{align*}
        x = x_1 g x_2.
        \end{align*}
        The element $e$ has a prefix of the form 
        \begin{align*}
             x_1g ( x_2 a x_1g)^! \byeq{\eqref{eq:swallow-idempotents}}  x_1g ( x_2 b x_1g)^! ( x_2 a x_1g)^!.
        \end{align*}
        The right side of the equation has $f$ as a prefix, and therefore $e$ and $f$ are prefix equivalent.
    \end{proof}
\end{proof}

A corollary of the above lemma, stated below, is that the map $a \mapsto a^!$ is a semigroup homomorphism, from the semigroup $A$ to the subsemigroup of its idempotents.

\begin{corollary}\label{cor:factorial-homomorphism}
    Let $A$ be a semigroup thaty satisfies~\eqref{eq:swallow-idempotents}.
    For every $a,b \in A$ we have 
    \begin{align*}
    (ab)^! = a^! b^!.
    \end{align*}
    In particular, a product of two idempotents is also an idempotent.
\end{corollary}
\begin{proof}
    Let us first establish that the product of two idempotents is an idempotent. Indeed, if $e$ and $f$ are idempotents, then 
    \begin{align*}
    ef \byeq{\eqref{eq:swallow-idempotents}} e(ef)^! f = (ef)^!,
    \end{align*}
    and therefore $ef$ is an idempotent. 
    
    Let us now prove the equality in the statement of the lemma. 
    The two elements in the equality are idempotents, with second element being an idempotent as a product of two idempotents. Also, they are in the same $\Jj$-class by~\eqref{eq:swallow-idempotents}. Finally, they have a common prefix (namely $a$) and a common suffix (namely $b$). Therefore they must be equal by Lemma~\eqref{lem:common-prefix-suffix}.
\end{proof}

The following lemma will be important in the proof. It will allow us to move an idempotent from the edges of a word to the internal part, as long as there is also another idempotent present nearby. 
\begin{lemma} 
    \label{lem:eaef}
    Assume the same assumptions as in the theorem.
    For every $a,e,f$ with $e$ and $f$ idempotents, 
\begin{align*}
eaf = eaef.
\end{align*}
\end{lemma}
\begin{proof}
    Decompose the idempotent $e$ into generators
    \begin{align*}
     e = e_1 \cdots e_n.
    \end{align*}
    We will show that 
    \begin{align}\label{eq:one-letter-of-idempotent}
    e a (e_i \cdots e_{n}f)^! =  e a (e_{i+1} \cdots e_{n}f)^! \qquad \text{for every $i \in \set{1,\ldots,n}$.}
    \end{align} 
    By combining all of these equalities, it will follow that 
    \begin{align*}
    e a f \justeq{by~\eqref{eq:one-letter-of-idempotent} applied to all $i \in \set{1,\ldots,n}$}
     ea(ef)^! \justeq{by Corollary~\ref{cor:factorial-homomorphism} } eaef 
    \end{align*}
    thus proving the lemma.
    
    Apply Claim~\ref{claim:multmat-tool} to: 
    \begin{align*}
    e & := e \\
    f & := (e_{i+1} \cdots e_n f)^! \\
    x & := e_i \\
    y & := \text{first letter of $(e_{i+1} \cdots e_n f)^!$} \\
    b & := \text{all but the first letter of $(e_{i+1} \cdots e_n f)^!$}\\
    a & := a 
    \end{align*}
    yielding 
    \begin{align*}
    e a (e_i b)^!  (e_{i+1} \cdots e_n f)^! = e a (e_{i+1} \cdots e_n f)^!.
    \end{align*}
    To complete the proof~\eqref{eq:one-letter-of-idempotent}, and thus also of the lemma, it remains to show that 
    \begin{align*}
         (e_i b)^!  (e_{i+1} \cdots e_n f)^! =  (e_i e_{i+1} \cdots e_n f)^!.
        \end{align*}
    Both sides of the equality are idempotents, with the left hand being idempotent because idempotents form a subsemigroup by Corollary~\ref{cor:factorial-homomorphism}. Both sides are $\Jj$-equivalent, since they are idempotents that are generated by $e_1,\ldots,e_n,f$. Finally, both sides have a common prefix, namely $e_i$ and both sides have a common suffix, namely $f$. Thefefore both sides are equal by Lemma~\ref{lem:common-prefix-suffix}.
\end{proof}



\begin{lemma}\label{lem:eae-hom}
    Assume the same assumptions as in the theorem. Then for every idempotent $e \in A$, the function $a \mapsto eae$ is a semigroup homomorphism of type $A \to eAe$.
\end{lemma}
\begin{proof} 
    Call an element $a \in A$ \emph{good} if 
    \begin{align*}
        eabe = eaebe
        \end{align*}
        holds for every $b,e \in A$ with $e$ idempotent. The lemma says that all element of $A$ are good. We will prove this by induction on the infix order. We begin with the following observation. 
    \begin{claim}
        \label{claim:good-products} A product of two good elements is also good.
    \end{claim}
    \begin{proof}
        Suppose that $a_1$ and $a_2$ are good. Then the product $a_1 a_2$ is als good because:
        \begin{align*}
            ea_1a_2be \justeq{because $a_1$ is good}
            ea_1ea_2be \justeq{because $a_2$ is good}
            ea_1ea_2ebe \justeq{because $a_1$ is good}
            ea_1a_2ebe.
            \end{align*}
    \end{proof}

    Therefore, in order to prove the lemma, it is enough to show that every generator $a$ is good. We need to show that 
\begin{align*}
eabe = eaebe 
\end{align*}
holds for every $b,e$ with $e$ idempotent.  
    Decompose $e$ as $e = x \bar  x$ where $x$ is some generator and $x \in A$ is prefix equivalent to $e$. 
    Consider a power of the matrix $\multmat \Sigma A$ that is divisible by $!$, and consider a line in this matrix which uses only the letter $x$, except for one position that is divisible by $!$ and which uses the letter $a$. Here is an example of two such lines:
    \mypic{6}
    We will show that we can find a column of the matrix (in red), which will distinguish the two lines if the conclusion of the lemma fails. This column is shown in the following picture:
    \mypic{5}
    When evaluated to together with the red column, the two lines give the results:  
    \begin{align}
        \label{eq:results-of-top-and-bottom-lines}
    \myunderbrace{ea (\bar x x)^! b e}{top line} 
    \quad 
    \myunderbrace{eabe}{bottom line}
    \end{align}
    Therefore, by the assumption that the matrix is finitary, we know that the two values in~\eqref{eq:results-of-top-and-bottom-lines} must be equal. To complete the proof of the lemma, it remains to show that the first of the two values, corresponding to the top line, is equal to $eaebe$. The only difference is that the first value uses $(\bar x x)^!$ instead of $e = (x \bar x)^!$. But this difference can easily be overcome:
    \begin{align*}
        eaebe \justeq{Lemma~\ref{lem:swallow-idempotents}} 
    eae(\bar x x)^! e be \justeq{Lemma~\ref{lem:eaef}} 
    ea(\bar x x)^!  be.
    \end{align*}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:finitary-generator}]
    We want to show that the semigroup is almost commutative, i.e.
    \begin{align*}
    abcd = acbd 
    \end{align*}
    holds for every $a,b,c,d \in A$. By the assumption $A^2 = A$, every element contains an idempotent, and therefore it is enough to show that the above equality holds whenever it is prepended and appended with some idempotents $e$ and $f$:  
    \begin{align*}
        eabcdf = eacbdf.
        \end{align*}
    Define $g = ef$. This is an idempotent by Corollary~\ref{cor:factorial-homomorphism}. By Lemma~\ref{lem:eaef}, the above equality is the same as 
    \begin{align*}
        gabcdg = gacbdg.
        \end{align*}
    By Lemma~\ref{lem:eae-hom}, the map $x \mapsto gxg$ is a semigroup homomorphism. The co-domain of this homomorphism, which is $gAg$, is a monoid. By the monoid case, we know that this monoid is commutative. Thus the above equality holds.         
\end{proof}


==> idempotent-good.tex <==
\section{Kleene star of good transductions}
\label{sec:idempotent-good}

In this section, we prove Lemma~\ref{lem:idempotent-good}. In the assumptions of this lemma, we have a finite semigroup  $A$, which satisfies the following conditions: 
\begin{enumerate}
    \item $A^2 = A$;
    \item for every $a \neq b \in A$ there exist $x,y \in A$ with $xay \neq xby$.
\end{enumerate}
We need to show that if a class $\Cc$ of surjective $A$-graphs is  the range of some good transduction, then also $\subalgebra \Cc$ is the range of some good transduction.


We do not yet know how to prove this lemma. We do know, however, how to prove it in the special case of monoids. 

==> invertible.tex <==
\section{Transductions that output trees}
\label{sec:transductions-that-output-trees}
In Section~\ref{sec:complexity-decreasinng}, we talked about transductions that input trees. In this section we talk about transductions that output trees. (Ideally, we would like to talk about transductions that output general trees, but so far we can only prove results for transductions that output trees of bounded height.) 

\begin{theorem}\label{thm:c-to-tree} Let $\alpha$ be a transduction that is complexity preserving, and whose outputs are trees of bounded height.  Then $\alpha$ is sub-definable.
\end{theorem}


For a tree, define its \emph{root pre-order} to be the pre-order that corresponds to the partition of the universe (the leaves of the tree) into the children of the root. If the root is node is ordered, then the root pre-order is a total pre-order (i.e.~a transitive relation such that every pair is related in at least one direction), and if the root node is unordered, then the root pre-order is an equivalence relation. The key behind the proof of the theorem is the following lemma, which says that the root pre-order of the input tree can be produced, by a sub-definable transduction, in the output structure.

% The main step in the proof of the above theorem will be the following lemma. 

% \begin{lemma}\label{lem:same-inputs}
%     Let $\varphi$ be a $\Cc$-to-tree transduction which is complexity preserving, and which has outputs of bounded height. Then there is a definable $\Cc$-to-tree transduction that is complexity preserving, whose outputs have bounded height, and whose inputs contain all inputs of $\varphi$.
% \end{lemma}

% Before proving the lemma, we use it to prove the theorem.
% \begin{proof}[Proof of Theorem~\ref{thm:c-to-tree} using Lemma~\ref{lem:same-inputs}] 
%     We will show that there is a definable $\Cc$-to-tree transduction $\psi$, which has outputs of bounded height, is complexity preserving, and whose inputs contain all inputs of the original transduction $\varphi$. Let $k$ and $\ell$ be the bounds on the heights of the output trees in $\varphi$ and $\psi$, respectively, and consider the following diagram:
%     \[
%     \begin{tikzcd}
%     \Cc 
%     \ar[r,"\varphi"]
%     \ar[rd,"\psi"']
%     &
%     \text{trees of height at most $k$}
%     \\
%     &
%     \text{trees of height at most $\ell$}
%     \ar[u,"\psi^{-1};\varphi"']
%     \end{tikzcd}
%     \]
%     By the assumption that the inputs of $\psi$ contain all inputs of $\varphi$, we know that the top arrow $\varphi$ is contained in the composition of the two bottom arrows $\psi$ and $\psi^{-1};\varphi$. The first bottom arrow $\psi$ is an \mso transduction. The second bottom arrow $\psi^{-1};\varphi$ is  complexity preserving (as the composition of two  complexity preserving transductions), and its inputs are trees, and therefore it is contained in an \mso transduction by Theorem~\ref{thm:complexity-decreasing}. Therefore, both bottom arrows are contained in \mso transductions, and thus the same must be true for the top arrow, which is contained in the composition of the bottom arrows.
% \end{proof}

% The rest of this section is devoted to proving Lemma~\ref{lem:same-inputs}. (todo: 4 pages using Factorization Forests)

\begin{lemma}\label{lem:root-order2}
    Let $\alpha$ be a transduction that is complexity preserving, and whose outputs are trees of bounded height.   Then 
    \begin{align*}
    \setbuild { (\structa,  (\structa, \le))}{$\le$ is the root order  for some $\structt$ with $(\structa,\structt) \in \alpha$ }
    \end{align*}
    is sub-definable.
\end{lemma}

Before proving the lemma, we use it to complete the proof of Theorem~\ref{thm:c-to-tree}. 

\begin{proof}[Proof of Theorem~\ref{thm:c-to-tree} using Lemma~\ref{lem:root-order}]
    We prove the theorem by induction on the maximal height of output trees. Since the height of output trees is bounded, this is legitimate finite parameter for the induction. The base case is when $k=0$, which means that outputs are trees with only one node, is trivial.  

    Consider the induction step. Suppose that the theorem is true for $k$, and consider a transduction $\alpha$ as in the assumption of the theorem where the maximal height of the output trees is $k+1$.  We will now show that the transduction that corresponds to $\alpha$ on its proper subtrees is complexity preserving. 
    
    \begin{claim}
        The following transduction is complexity preserving
        \begin{align*}
            \beta = \setbuild{ (\structa|U, \structt|U)}{$(\structa, \structb) \in \alpha$ and $U$ is a proper subtree of $\structt$ }.
            \end{align*}
    \end{claim}
    \begin{proof}
        The following quantities are asymptotically equivalent, where $(\structa,\structt)$ ranges over $\alpha$,  $U$ ranges children of the root of $\structt$, and $W$ ranges over subsets of $U$:
        \begin{align*}
        \mu(\structt|U, W) \sim \mu(\structt, W) \sim \mu(\structa,W) \sim \mu(\structa|U, W).
        \end{align*}
        In the  middle equivalence we use the assumption on $\alpha$, while in the first and last equivalences, we use the fact that subtrees have constant complexity.         
    \end{proof}

    Since the transduction in the above claim has smaller height of output trees than $\alpha$, we can use the  induction assumption from the theorem to conclude that it  is sub-definable.  Apply Lemma~\ref{lem:root-order} to $\alpha$, yielding a sub-definable transduction $\gamma$ that produces for every input $\structa$ all possible root pre-orders.  The \mso transduction that witnesses sub-definability of $\alpha$ works as follows: first run $\gamma$ to compute the root pre-order, and then for every equivalence class of the root pre-order, execute the transduction from the claim. 
\end{proof}


    The rest of Section~\ref{sec:transductions-that-output-trees} is devoted to proving Lemma~\ref{lem:root-order}. 
    Without loss of generality we assume that either: (a) in all input trees to $\alpha$, the root node is unordered; or (b) in all inputs trees to $\alpha$, the root node is ordered. This is because  the every transduction that inputs trees can be decomposed into a union of two transductions, one satisfying (a) and the other satisfying (b), and the lemma can then be applied separately to the two transductions. The two cases are treated in Sections~\ref{sec:root-is-unordered} and~\ref{sec:root-is-ordered}.

    \subsection{The root node is unordered}
    \label{sec:root-is-unordered}

    In this section, we prove Lemma~\ref{lem:root-order} for a transduction $\alpha$ in which all output subtrees have an unordered root node. In this case, the root pre-order is an equivalence relation. For the rest of this section, when speaking of \emph{the root equivalence relation} in a tree $\structt$, which will be referring to this equivalence relation.  

    We say that a set $X$ \emph{cuts} a set $Y$ if at least one element of $Y$ is in $X$ and at least one element of $Y$ is not in $X$.  Ideally we would like to know which sets do not cut any equivalence classes, such sets are consistent with the equivalence relation. In a first step, we will show that we can at least approximate the number of cuts. 



    \begin{claim}\label{claim:commutative-approximation} There exists an \mso formula $\varphi(X)$ over the vocabulary of the input structures in $\alpha$, a commutative semigroup $A$ and  some $k \in \set{1,2,\ldots}$ with the following property. For every $(\structa,\structt) \in \alpha$:
        \begin{enumerate}
            \item \emph{sound:} if $X \subseteq \structa$ cuts zero root equivalence classes of $\structt$, then  $\structa \models \varphi(X)$.
            \item \emph{complete:} if $X \subseteq \structa$ cuts at least $k$ root equivalence classes of $\structt$, then $\structa \not \models \varphi(X)$.
            \item \emph{homogeneous:} for every root equivalence class $U$ of $\structt$ there is a function 
            \begin{align*}
                h_U : \powerset U \to A
            \end{align*}
            such that for every subset $X \subseteq \structa$, whether  $\structb \models \varphi(X)$ holds depends only on the product, in the commutative semigroup $A$, of the semigroup elements $h_U(X \cap U)$, with the product ranging over root equivalence classes $U$.
        \end{enumerate}
    \end{claim}
    \begin{proof}
        If a set $X \subseteq \structt$ cuts no equivalence classes in $\structt$, then its complexity in $\structt$ is bounded, which yields some  $\ell_0$ that makes the following implication true: 
        \begin{enumerate}
            \item[(a)]  if $X$ cuts no root equivalence classes, then the  complexity of $X$ in $\structt$ is $\le \ell_0$.
        \end{enumerate}
        Using the assumption that the transduction $\alpha$ is complexity preserving, we know that there are constants $\ell_1$ and $\ell_2$ such that every subset $X$ of the universe satisfies:  
        \begin{enumerate}
            \item[(b)] if the complexity of $X$ in $\structt$ is $ \le \ell_0$, then the complexity of $X$ in $\structa$ is $\le \ell_1$;
            \item[(c)]if the complexity of $X$ in $\structa$ is $ \le \ell_1$, then the complexity of $X$ in $\structt$ is $\le \ell_2$.
        \end{enumerate}
        A set of constant complexity  in a tree can only cut a bounded number of root equivalence classes, which yields some $k$ such that 
        \begin{enumerate}
            \item[(d)]  if the complexity of $X$ in $\structt$ is $ \le \ell_2$, then it cuts  $\le k$ root equivalence classes. 
        \end{enumerate}
            
        Define $\varphi(X)$ to be the property: the logical complexity of $X$ inside $\structa$ is at most $\ell_1$. This is an \mso formula, since logical complexity can be described in \mso.  Conditions (a) and (b) give the soundness condition from the claim, while conditions (c) and (d) give the completeness condition. 
        It remains to prove the last condition in the claim, about the semigroup. 
        

        (fill in about the last condition)
    \end{proof}

    Apply the above claim, yielding some formula $\varphi$, some semigroup $A$ and some number $k$.
    For a pair $(\structa,\structt) \in \alpha$ and a root equivalence class $U$, define its \emph{full type} to be the semigroup element obtained by applying the function $h_U$ from Claim~\ref{claim:commutative-approximation} to the full set $U$, and define its \emph{empty type} to be the result of applying $h_U$ to the empty set. Define the profile of the root equivalence class to be the pair of semigroup elements (full type, empty type). 
    
    We will show that for every  fixed profile, there is a sub-definable transduction which produces equivalence classes of a given profile. More formally, we will show that for 
    every $a,b \in A$ the following transduction is sub-definable
    \begin{align}\label{eq:profile-subtransduction}
        \setbuild{
        (\structa, \text{family of root equivalence classes of profile $(a,b)$})
        }
        {$(\structa,\structt) \in \alpha$}.
        \end{align}
    By aggregating the outputs of these transductions for the finitely many possible profiles, we will get the family of all root equivalence classes, as required in the lemma. 
    It remains to describe the sub-definable transduction in~\eqref{eq:profile-subtransduction}. 
    
    \paragraph*{The transduction for a given profile.}
    Fix a profile $(a,b)$ for the rest of this proof.  Our goal is to show that the transduction~\eqref{eq:profile-subtransduction} is sub-definable. We will only care about pairs $(\structa, \structt)\in \alpha$ in which there are at least two equivalence classes of the fixed  profile.  Indeed, for pairs which have only one root equivalence class, the output can easily be given by a sub-definable transduction, which simply guesses the unique equivalence class.  

    In the proof, we will only work with the elements that belong to equivalence classes of profile $(a,b)$; let us write $W$ for this subset.  (This subset depends on the choice of $(\structa,\structt)$, but we assume this choice to be implicit from the context, so we do not write it.)
    In the remainder of the proof, we will use the following technical definition.  
    We say that a set  $X$ is a \emph{seed} for  a pair $(\structa, \structt) \in \alpha$ if it is a subset of the universe in the corresponding structures, and  it satisfies all the following conditions:
    \begin{enumerate}
        \item \label{it:maximal-commutative-phi} $X$ satisfies $\varphi$ and is contained in $W$;
        \item \label{it:maximal-commutative-full} there is some root equivalence class of profile $(a,b)$ that is contained in $X$;
        \item \label{it:maximal-commutative-empty} there is some root equivalence class of profile $(a,b)$ that is disjoint with $X$;
        \item \label{it:maximal-commutative-maximal} the number of root equivalence classes cut by $X$ is  maximal, among sets $X$ that satisfy all the conditions~\ref{it:maximal-commutative-phi}, \ref{it:maximal-commutative-full}, \ref{it:maximal-commutative-empty}.
    \end{enumerate}

    \begin{claim}
        If $(\structa,\structt)\in \alpha$ has at least two classes of profile $(a,b)$, then it has a seed. 
    \end{claim}
    \begin{proof}
        It is enough to show that there is some  set $X$ that satisfies the first three conditions in the definition of a seed; this will imply that there is also some subset which furthermore satisfies the last maximality condition. To see why some set satisfies the first three conditions, recall the  completeness condition in Claim~\ref{claim:commutative-approximation}. This completeness ensures that $\varphi$ selects every set that does not cut any root equivalence classes; in particular we can choose a set that selects one equivalence class with profile $(a,b)$ and rejects the remaining equivalence classes.  (Here we use the assumption that there are at least two root equivalence classes of the profile $(a,b)$.)        
    \end{proof}


    Let $X$ be a seed, and  let $U_1,\ldots,U_\ell$ be the root equivalence classes that are cut by this seed. Observe that $\ell$ is at most the bound $k$ from Claim~\ref{claim:commutative-approximation}, since this is the maximal number of root equivalence classes that can be cut by a set that satisfies $\varphi$.  The main observation is in the following claim, which shows that the equivalence classes in $W$ can be determined by looking are sets that are similar to a seed. 
    
    \begin{claim}\label{claim:seed-separator}
        Let $X$ be a seed, and let $x, y \in W \setminus (U_1,\ldots,U_\ell)$. Then $x$ and $y$ are in the same equivalence class if and only if they can be separated by a set $Y$ satisfying: 
\begin{enumerate}
    \item[(*)] $Y$ is contained in $W$, satisfies $\varphi$, and agrees with $X$ on $U_1 \cup \cdots \cup U_\ell$.
\end{enumerate}
    \end{claim}
    \begin{proof}
        By the  maximality condition in  a seed, if a set $Y$  satisfies (*), then it cannot cut any equivalence class other than $U_1,\ldots,U_\ell$. Therefore, if $x$ and $y$ can be separated by a set satisfying (*), then they are in the same equivalence class. 

        We now prove the other implication -- for $x,y \in W \setminus (U_1 \cup \cdots \cup U_\ell)$, if $x$ and $y$ are in  the same equivalence class,  then they can be separated by a set satisfying (*). The idea is the following. By definition, the seed $X$ is empty on some class from $W$ and full for some other class. However, since all classes in $W$ have the same profile, we could choose the empty class and the full class arbitrarily while keeping $\varphi$ true.  In particular the empty class could be the one of $x$ and the full class could be the one of $y$, thus separating the two elements. 
    \end{proof}

    From the above claim we get the transduction. The transduction guesses the sets $U_1,\ldots,U_\ell$, with $\ell$ being a bounded number, as well as the set $W$, and then it defines the partition of $W$ according to Claim~\ref{claim:seed-separator}: two elements are in the same class if they cannot be separated by a set satisfying (*). This is sub-definable, since condition (*) can be defined in \mso once the parameters $U_1,\ldots,U_\ell$ and $W$ are known. 
\subsection{The root node is ordered}
\label{sec:root-is-ordered}


\begin{claim}\label{claim:non-commutative-approximation} There exists an \mso formula $\varphi(X)$ over the vocabulary of the input structures in $\alpha$, a (not necessarily commutative)  semigroup $A$ and  some $k \in \set{1,2,\ldots}$ with the following property. For every $(\structa,\structt) \in \alpha$:
    \begin{enumerate}
        \item \emph{sound:} if $X \subseteq \structa$ is a prefix of the root order in  $\structt$, then  $\structa \models \varphi(X)$.
        \item \emph{complete:} if $X \subseteq \structa$ alternates at  $k$ times in the root order  of $\structt$, then $\structa \not \models \varphi(X)$.
        \item \emph{homogeneous:} for every root equivalence class $U$ of $\structt$ there is a function 
        \begin{align*}
            h_U : \powerset U \to A
        \end{align*}
        such that for every subset $X \subseteq \structa$, whether  $\structb \models \varphi(X)$ holds depends only on the product, in the commutative semigroup $A$, of the semigroup elements $h_U(X \cap U)$, with the product ranging over root equivalence classes $U$, ordered according to the root order.
    \end{enumerate}
\end{claim}

==> matrices.tex <==
\subsection{Matrices of finite order}

\begin{definition}
    Let $A$ be a semigroup. A \emph{matrix over $A$} is any function 
    \begin{align*}
    M : X \times Y \to A
    \end{align*}
    for some finite sets $X$ and $Y$.
\end{definition}

\begin{definition}
    For two matrices over the same semigroup $A$,
    \begin{align*}
        M_i : X_i \times Y_i \to A \qquad \text{for $i=1,2$},
        \end{align*}
    their \emph{Kronecker product} is the matrix denoted by $M_1 \otimes M_2$, in which the rows are $X_1 \times X_2$, the columns are $Y_1 \times Y_2$, and the cells are  defined by 
    \begin{align*}
    ((x_1,x_2), (y_1,y_2)) \quad \mapsto \quad \myunderbrace{M_1(x_1,y_1) \cdot M_2(x_2,y_2)}{product in the semigroup $A$}.
    \end{align*}
\end{definition}
Two matrices are called \emph{isomorphic} if they are the same, up to renaming the rows of columns. One can easily see that the Kronecker product is associative up to isomorphism of matrices. Since we identify isomorphic matrices, we will think of the Kronecker product as being simply associative. 
The $n$-th \emph{Kronecker power} of a matrix $M$ is the result of multiplying the matrix by itself $n$ times.
\begin{align*}
M^{\scriptsize{\encircle n}} \eqdef \myunderbrace{M \otimes \cdots \otimes M}{$n$ times}
\end{align*}


In the proof, we will frequently be looking at sub-matrices, as defined below. 
\begin{definition}
    Let $M,N$ be two matrices over the same semigroup. We say that $M$ is a \emph{sub-matrix} of $N$, written as $M \le N$, if $M$ is isomorphic to matrix that can be obtained from $N$ by removing rows and columns.We say that two matrices are \emph{equivalent} if they one is a sub-matrix of the other and vice-versa.
\end{definition}

It is not hard to see that the Kronecker product respects the sub-matrix ordering, 
\begin{align*}
M_1 \le N_1, M_2 \le N_2 \qquad \Rightarrow \qquad M_1 \otimes M_2 \le N_1 \otimes N_2.
\end{align*}
In particular, equivalence of matrices is a congruence with respect to Kronecker product. 


\begin{definition}[Kronceker semigroup]
    Let $A$ be a semigroup. The \emph{Kronecker semigroup of $A$}, denoted by   $\kronecker{A}$ to be the semigroup where the elements are matrices modulo equivalence, and the semigroup operation is Kronecker product.
\end{definition}

We say that a matrix $M$ over some semigroup $A$ has \emph{finite order} if 
it generates a finite sub-semigroup of the Kronecker semigroup. In other words, a matrix has finite order if and only if the set of its Kronecker powers is finite, up to matrix equivalence. 

\begin{theorem}
    Let $A$ be a monoid, and let $M$ be a matrix over $A$ which contains the monoid unit $1 \in A$. Then $M$ has finite order if and only if it is equivalent to a  multiplication matrix $\multmat B C$ where $B,C \subseteq A$ are unipotent subsets that commute with each other:
    \begin{align*}
    \forall b \in B \forall c \in C \quad bc = cb.
    \end{align*}
\end{theorem}
\begin{proof}
    The right-to-left implication is clear, so we focus on the left-to-right implication. This will follow from the following claim, which treats the left-to-right implication for $2 \times 2$ matrices.
    
    \begin{claim} Consider a unipotent matrix of dimension $2 \times 2$ of the form 
        \begin{align*}
            \begin{array}{c|cc}
                 & \text{left} & \text{right} \\
                \hline
                 \text{up} & 1 & b \\
                \text{down} & c & d
            \end{array}
            \end{align*}
        Then $d = bc =cb$.
    \end{claim}
    \begin{proof} Let $M$ be the matrix from the assumption of the claim.  Consider the $n$-th Kronecker power of $M$. For $i \in \set{1,\ldots,n}$, define the \emph{$i$-th singleton row} to be the row which has ``up'' everywhere except for the $i$-th position:
        \begin{align*}
        \myunderbrace{\text{up}, \ldots, \text{up}, \text{down}, \text{up}, \ldots, \text{up}}{there is only one down, at the $i$-th position}.
        \end{align*}
        Similarly we define the $i$-th singleton column, it uses left everywhere except for the $i$-th position where it uses right. If we pair the $i$-th singleton row with the $j$-th singleton column, then the corresponding cell in the $n$-th Kronecker power of $M$ is: 
        \begin{align*}
        \begin{cases}
            bc & \text{if $i<j$} \\
            d & \text{if $i=j$} \\
            cb & \text{if $i > j$}
        \end{cases}
        \end{align*}
        Suppose now that $bc \neq d$. In this case, if $i < j$ then the corresponding singleton rows can be distinguished by the $j$-th singleton column, and therefore all the singleton rows are different. If $cb \neq d$, then the corresponding singleton rows can be distinguished by the $i$-th singleton column, and thus again al singleton rows are different. Summing up, if one of the equalities in the conclusion of the claim is violated, then the $n$-th Kronecker power of the matrix has at least $n$ distinct rows, and thus the matrix has infinite order. 
    \end{proof}
    
    The general case follows from the $2 \times 2$ case. Indeed, for the names of the columns we can use the row that contains 1, and for the names of the rows we can use the column that contains 1. By the equalties from the claim, the remaining cells in the matrix arise as in a multiplication matrix, and a commutative one at that. 
    \end{proof}

==> monoids.tex <==
\section{Monoids}

\begin{definition}
    A hypergraph is a tuple that consits of:
    \begin{enumerate}
        \item a set $A$ of \emph{output colours};
        \item a set $V$ of vertices, with each vertex $v$ having an associated set $A_v$ of \emph{input colours};
        \item a \emph{hyperedge colouring}, which is a function of type
            \begin{align*}
                \prod_{v \in V} A_v \to A.
            \end{align*}
    \end{enumerate}
\end{definition}

For example, a hypergraph with two vertices called ``rows'' and ``colums'' is the same thing as a matrix of the set of output colours. 

Consider a hypergraph $G$ and a tree family $\Tt$. Define the 

\begin{definition}
    A \emph{tree decomposition} of a hypergraph $G$ is a tree together with:
    \begin{enumerate}
        \item a labelling which assigns to each node $x$ a hypergraph $G_x$;
        \item a bijection of the leaves of the tree with the vertices of $G$;
    \end{enumerate}
    subject to the following conditions:
    \begin{enumerate}
        \item for every leaf $x$, the hypergraph $G_x$ has one vertex, the input and output colours in $G_x$ are the same as the input colours of $x$ in $V$;
        \item the ouptut colours of the hypergraph 
        \item every tree node $x$ is labelled a hypergraph $G_x$ where: 
            \begin{enumerate}
                \item if $x$ is the root, then the output colours of $G_x$ are the same as in $G$;
                \item if $x$ is a leaf, then 
            \end{enumerate}
    \end{enumerate}
\end{definition}





\begin{theorem} 
    Let $A$ be a monoid, and let 
    \begin{align*}
    \Sigma \subseteq \setbuild{G}{$G$ is a one vertex graph over $A$, whose set of ouptut colours is unipotent }.
    \end{align*}
    Then the class of hypergraphs $\subalgebra \Sigma$ is good.
\end{theorem}
\begin{proof}
    Induction on the size of $\Sigma$. 
    
    Consider first the induction basis, where $\Sigma$ conains only one hypergraph $G$ with image $B \subseteq A$. Suppose first that the multiplication matrix $\multmat B B$ has finite order. In this case, $B$ commutes with itself, and therefore the monoid generated by $B$ is commutative. In this case, the appropriate tree decomposition is a star with unordered children. Otherwise, the matrix $\multmat B B$ has infinite order. In this case, the appropriate tree decomposition is a star with ordered children. To prove that this tree decomposition is appropriate, consider 


    Consider now the induction step. 
    \begin{itemize}
        \item Suppose first that there is some partition of $\Sigma$ into two disjoint sets $\Sigma_1$ and $\Sigma_2$, such that the two subsets 
        \begin{align*}
        \bigcup_{G \in \Sigma_1} \text{image of $G$}
        \qquad \text{and} \qquad 
        \bigcup_{G \in \Sigma_2} \text{image of $G$}
        \end{align*}
        commute. In this case, the tree decompositions are defined as follows. A graph $G_1 \cdots G_n$ is mapped to the tree $(T_1,T_2)$ where $T_i$ is obtained by restricting the string $G_1 \cdots G_n$ to the letters from $\Sigma_i$, and applying the tree decompositions for the class  $\subalgebra{\Sigma_i}$. Let us prove this function is good.
        \begin{align*}
        \text{rank of $U$ in $T(G)$} 
        \quad \stackrel {\substack{G \in \subalgebra \Sigma \\ U \subseteq \text{vertices of }G}} \preceq \quad 
          \text{rank of $U$ in $G$}
        \end{align*}
        Suppose then that $\Xx$ is a family of pairs $(G,U)$ which makes the left side unbounded. This means that either: 
    \end{itemize}
\end{proof}




==> rubbish.tex <==

number of equivalence classes that contain elements of both $U$ and its complement. 

We now describe a rank measure that is asymptotically equivalent to logical rank over trees of bounded height. For a tree $T$ and distinguished node $x$, define the \emph{local structure} to be the structure where the universe is the set of descendants of the distinguished node, and in which the structure is:
\begin{enumerate}
\item if the distinguished node is unordered, then there is an equivalence relation corresponding to the partition into the child subtrees;
\item if the distinguished node is ordered, then there is a linear quasi-order corresponding to the ordered partition into child subtrees;
\end{enumerate}
Define the tree the \emph{tree rank} of a set of leaves $U$ in a tree $T$ to be the maximum, ranging over nodes $x$ of the tree, of the logical rank of the subset $U$ restricted to the local structure at $x$. Instead of logical rank, we could have used the measures defined in Examples~\ref{ex:quasi-linear-orders} and~\ref{ex:equivalence-relations}, and the resulting tree rank would be the same up to asymptotic equivalence. One can show without difficulty that if a class of trees has bounded height, then logical rank is asymptotically equivalent to tree rank. 

\begin{definition}[Equivalent set functions]
    Two set functions $\mu_1$ and $\mu_2$ over the same class of structures $\Cc$ are called \emph{equivalent} if they are asymptotically equivalent:
    \begin{align*}
    \boundeq
    {\mu_1(\structa,U)}
    {\structa \in \Cc \\
    U \subseteq \structa}
    {\mu_2(\structa,U)}.
    \end{align*}
   \end{definition}
   
   In this paper, we will be primarily interested in set functions which compute the rank of some matrix. The matrices that we consider in this paper are very general, and they do not need to use values from a field. 
   
   \begin{definition}[Matrix]
    A \emph{matrix} is any function of type 
    \begin{align*}
    \myunderbrace{A_1}{this set is \\ called the \\ \emph{columns}} 
    \qquad 
    \times
    \qquad 
    \myunderbrace{A_2}{this set is \\ called the \\ \emph{rows}}
    \qquad 
    \to
    \qquad 
    \myunderbrace{A}{this set is \\ called the \\ \emph{values}}.
    \end{align*} 
    The rows, columns, and values are all required to be finite sets.
   \end{definition}
   The set $A$ of values need not be a field. The \emph{row rank} of a matrix is defined to be the number of distinct rows, i.e.~the number of rows that can be distinguished by some column. Likewise we define the \emph{column rank}. If the set of values $A$ is assumed to be fixed, the row rank and column rank are bounded by each other.
   
   \begin{fact}\label{fact:row-column}
    For every fixed set of values $A$, row rank and column rank are asymptotically equivalent:
    \begin{align*}
    \boundeq
    {\text{row rank of $M$}}
    {M : A_1 \times A_2 \to A}
    {\text{column rank of $M$}}.
    \end{align*}
   \end{fact}
   
   
   
   
   
   
   \begin{definition}[Structure]\label{def:structure}
    A structure consists of a set $U$, called the \emph{universe} of the structure, together with finitely many unary predicates that take set arguments
    \begin{align*}
    R_1,\ldots,R_n \subseteq \powerset U.
    \end{align*} 
   \end{definition}
   
   One could imagine a more general notion of structure, which allows binary relations on elements, or binary relations on sets, etc. As far as the results in this paper as concerned, the general case is already captured by structures in which there is a single relation $R \subseteq \powerset U$, see~\cite[Lemma B.3]{DBLP:journals/corr/abs-2305-18039}.
   
   
   
   One could consider other representations, where the universe also has elements for the nodes of the tree, but we do not use such representations in this paper. 
in several ways: 
\begin{enumerate}
    \item the universe is $V$, and the family $\Tt$ is represented as a relation that takes one argument of set type;
    \item the 
\end{enumerate}
The trees that we use in this paper are rooted, unranked, and partially ordered. By partially ordered we mean that for some nodes (called \emph{commutative nodes}), there is a no order on the children, and for the remaining nodes (called \emph{non-commutative nodes}) there is a total order on the children. These are the only two alternatives, i.e.~no order or a total order. One could imagine intermediate kinds of stucture, e.g.~a tree order or a cyclic order, but we do not use those intermediate kinds. 



\begin{definition}[Tree]\label{def:tree}
 A \emph{partially ordered tree} is defined to be:
 \begin{itemize}
 \item an \emph{unordered tree}, i.e.~a connected acyclic undirected graph with a distinguished root node (we use the usual tree terminology, as parent, child, ancestor, descendant, leaf and sibling);
 \item a distinguished subset of \emph{ordered nodes} in the tree from the first item;
 \item for each ordered node, a corresponding \emph{child order}, which is a linear order on its children.
 \end{itemize}
 We assume that there are no unary nodes in a tree, i.e.~every node is either a leaf or has at least two children.
\end{definition}

From now on, we simply say \emph{tree} instead of partially ordered tree. 
An unordered tree can be seen as a special case of a tree, in which none of the nodes are ordered. An \emph{interval} in a tree is a set of nodes that has one of the following two types:
\begin{itemize}
\item \emph{ordered interval}: an interval in the child order of some ordered node;
\item \emph{unordered interval}: any subset of children for some unordered node.
\end{itemize}
A \emph{subforest} in a tree is any set of leaves that is obtained by taking some set of siblings, and returning all leaves that are descendants of it. 

\begin{lemma}\label{lem:tree-subforests}
 A tree is uniquely determined by its subforests.
\end{lemma}


==> trash <==


\begin{corollary}
    Assume that a semigroup $A$ satisfies~\eqref{eq:swallow-idempotents}. Then
\begin{enumerate}
    \item The idempotents of $A$ form a sub-semigroup.
    \item The semigroup of idempotents is almost commutative.
    \item The function $a \mapsto a!$ is a semigroup homomorphism from $A$ to the semigroup of its idempotents described in the previous item.
\end{enumerate}
\end{corollary}
\begin{proof}\ \\
    \begin{enumerate}
        \item Let us first show that the product of two idempotents is an idempotent. Suppose that $e$ and $f$ are idempotents. Then $ef$ is an idempotent, since it is equal to the idempotent $(ef)!$ as explained below:
        \begin{align*}
        ef & = \justifyeq{appplying~\eqref{eq:swallow-idempotents} to the idempotent $(ef)!$  generated by $e$ and $f$}\\
        e(ef)!f & = \justifyeq{because $e$ and $f$ are idempotents} \\
        (ef)!
        \end{align*}

        \item Consider four idempotents $a,b,c,d$. Then
        \begin{align*}
        abcd & = \justifyeq{because idempotents form a subsemigroup}\\
        abcbcd & = \justifyeq{because~\eqref{eq:swallow-idempotents} implies that $abc=acbc$ and $bcd=bcbd$}\\
        acbc bcbd & = \justifyeq{because $bc$ is an idempotent} \\
        acbd,
        \end{align*}
        which proves that the semigroup of idempotents is almost commutative.
        \item  same
        \begin{align*}
            a!b! & = \justifyeq{by `'\eqref{eq:swallow-idempotents}} \\
            a!(ab)! b!
        \end{align*}
    \end{enumerate}
\end{proof}


\begin{lemma} 
    \label{lem:eaef}
    If $e,f$ are idempotents and $a \le e$ or $a \le f$ then 
\begin{align*}
eaf = eaef.
\end{align*}
\end{lemma}
\begin{proof}
    By symmetry, we assume that $a \le e$.
    We first show that for every $a \le e$, we have 
    \begin{align}
        \label{eq:regularize}
        eae = ea^{!+1}e.
    \end{align}
    By $A = A^2$, we know that $a$ must begin or end with an idempotent. By symmetry, assume that $a$ ends with an idempotent, i.e.~$af = a$ for some idempotent $f$. Then 
    \begin{align*}
    e  a^{!+1} e = e a f a^{!} e \byeq{\eqref{eq:swallow-idempotents}} eafe  = eae.
    \end{align*}

    The following claim shows that if we take an element of the $\Jj$-class of $e$ which begins and ends with idempotents (possibly strictly smaller than $e$), then its $\Hh$-class is uniquely determined by these idempotents.
\begin{claim}  Supposde that $a \sim e$ begins with an idempotent $e_1$ and ends with an idempotent $e_2$ (the idempotents $e_1$ and $e_2$ may be strictly smaller than $e$). Then   
        \begin{align*} 
 a  \hsim e_1 e a_2.
        \end{align*}
    \end{claim}
    \begin{proof}
        By~\eqref{eq:swallow-idempotents}, the element $e_1 a e_2$ is in the same $\Jj$-class as $e$. We have 
        \begin{align*}
        e_1 e e_2 \byeq{\eqref{eq:swallow-idempotents}} e_1 (e_1ae_2)^! e e_2, 
        \end{align*}
        and therefore $e_1 e e_2$ has $a$ as a prefix. By a symmetric argument, $e_1 e e_2$ also has $a$ as a suffix. Therefore, the two elements are $\Hh$-equivalent. 
    \end{proof}

    By the above claim, we know that if $a \le e$, then $eaf$ is in the same $\Hh$-class as $ef$. This $\Hh$-class is a group, and its identity is the idempotent $ef$. Therefore,
    \begin{align*}
    eaf  & = \justifyeq{because $ef$ is the identity in its $\Hh$-class}\\
    efeafef & = \justifyeq{by~\eqref{eq:regularize}} \\
    efea^{!+1}fef & = \justifyeq{becaue $a^! f = a^! fe$ by~\eqref{eq:swallow-idempotents}}\\
    efea^{!+1}efef & = \justifyeq{by~\eqref{eq:regularize}} \\
    efeaefef   & = \justifyeq{because $ef$ is the identity in its $\Hh$-class}\\
    eaef  
    \end{align*}
\end{proof}

\begin{corollary} For every idempotent $e$, the function 
    \begin{align*}
    a \mapsto eae
    \end{align*}
    is a homomorphism from the semigroup $\jdown e$ to the group of $e$. 
\end{corollary}
\begin{proof}
    \begin{align*}
    eabe \justeq{because $be$ is in the regular $\Jj$-class of $e$}
    ea(be)^{!+1}  \justeq{Lemma~\ref{lem:eaef}} 
    eae(be)^{!+1} \justeq{because $be$ is in the regular $\Jj$-class of $e$} 
    eaebe &
    \end{align*}
\end{proof}

\begin{lemma} 
    Let $a_1,\ldots,a_n \in A$ be such that the product $a = a_1 \cdots a_n$ is regular. Let $e = a^!$ and let $h$ be the homomorphism from the previous lemma. Then 
    \begin{align*}
        a = eh(a_1 \cdots a_n)e.
    \end{align*}
    be such that the products of both $a_1 \cdots a_n$ and $b_1 \cdots b_n$ are in the same regular $\Jj$-class. Let $e$ be the idempotent 
    \begin{align*}
    e = (a_1 \cdots a_n b_1 \cdots b_n)^!
    \end{align*}
    and let $h$ be the homomorphism $a \mapsto eae$. Then 

    \begin{align*}
    a_1 \cdots a_n \sim b_1 \cdots b_n \sim e
    \end{align*}
\begin{align*}
ea_1 \cdots a_n = e a_1 e a_2 e \cdots e a_n f
\end{align*}
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}
    If $e$ is an idempotent and $a \le e$, then $eaf = ea!af$. 
\end{lemma}
\begin{proof}
    Suppose first that $a$ ends with an idempotent, say $ag = a$ for some idempotent $g$. Then 
    \begin{align*}
    eaf = eagf = 
    \end{align*}
    \begin{align*}
    ea!af = ea!gef = egef 
    \end{align*}
\end{proof}

\begin{theorem}
    If 

    \begin{enumerate}
        \item Every finite class of hypergraphs.
        \item Let $M : A_1 \times A_2 \to A$ be an irredundant matrix. 
        \item Let $A$ be a semigroup with the following properties:
        
        For such a semigroup $A$, we have the operation
        \begin{align*}
        \myunderbrace{\Cc}{any class of\\ $A$-hypergraphs}
        \qquad \mapsto \qquad 
        \myunderbrace{\setbuild{ G_1 \cdots G_n}{$G_1,\ldots,G_n \in \Cc$}}{we call this class $\subalgebra \Cc$}
        \end{align*}
        \end{enumerate}
\end{theorem}

A \emph{decomposition}  is a sibling-ordered tree $T$ with the following structure:
\begin{enumerate}
    \item Every node is labelled by a finite set, called the \emph{colours at the node};
    \item In  every leaf, there are exactly two colours, ``yes'' and ``no''.
    \item For every non-leaf node $x$ there is a surjective  multiplication operation  
    \[
    \begin{tikzcd}
        \text{colours of $x_1$} \times \cdots \times \text{colours of $x_n$}
        \ar[r,"f"] & \text{colours of $x$}
    \end{tikzcd}
    \]
\end{enumerate}
For a set $X$ of leaves in the decomposition, and a node $x$, the \emph{colour of $X$ at node $x$} is defined by induction on the node $x$ as follows. If $x$ is a leaf, then the colour is ``yes'' or ``no'', depending on whether $x$ belongs to the set $X$. If $x$ is not a leaf, then the colour is defined by applying the multiplication operation to the colours at the children. A decomposition  defines a hypergraph, where the  vertices are the leaves and the colour of a subset of leaves is its colour (according to the decomposition) at the root. 

Here are the properties of decompositions that will be of interest to us: 
\begin{enumerate}
    \item A decomposition is called \emph{minimal} if for every node $x$ and every two different colours $c_1$ and $c_2$ at this node, there exist sets of leaves $X_1$ and $X_2$ that have different colours at the root, and colours $c_1$ and $c_2$ at the node $x$. This means that all colours can be differentiated at the root. 
    \item The \emph{order} of a decomposition is the height of the tree plus the maximal height of a set of colours used in nodes. We will be interested in decompositions of constant order. 
    \item If a node in a decomposition has many children, then its multiplication operation can be very complex. One way to limit this is to require that this multiplication operation arises from a certain semigroup, as defined below. A decomposition is called \emph{algebraic} if for every node  $x$ with at least 3 children $x_1,\ldots,x_n$ (such a node is  called \emph{semigroup node}) then 
        \begin{align*}
        \text{colours at $x$} = 
        \text{colours at $x_1$} = 
        \cdots
        \text{colours at $x_n$},
        \end{align*}
        and this set of colours can be equipped with a semigroup structure, such that the multiplication operation is the semigroup operation.
  \item A set $U$ of leaves is called $k$-consistent with a decomposition $T$ if for every node $v$ of the decomposition, one can partition the sequence of children of $v$ into at most $k$ intervals, such that every interval either saturated (i.e.~all of the leaves that are descendants of the interval have the same membership in $U$) or contains one child.
   Let $\alpha : \Nat \to \Nat$. A decomposition is called \emph{$\alpha$-consistent} if for every subset $X$ of leaves, we have 
  \begin{align*}
    \text{$T$-crossing of $X$} \le \alpha(\text{rank of $X$})
  \end{align*}
    

\end{enumerate}

Observe that if a decomposition is minimal, then it has no unary nodes (assuming that we remove unary nodes where the multiplication operation is a bijection between the colours of the parent and the colours of the child). A tree without unary nodes can be viewed as a family of subsets of the leaves, as described in the following definition.






\begin{lemma}
    If $\Cc$ is a class of hypergraphs of bounded linear width, then there is some $k$ such that every hypergraph in $\Cc$ arises from some decomposition that is algebraic, minimal, and has order at most $k$. 
\end{lemma}
\begin{proof}
    We prove the lemma in two steps. First, we use the factorisation forest theorem of Simon to show that every hypergraph arises from some decomposition that is algebraic and of bounded order, but not necessarily minimal. Then we make these decompositions minimal. 
\end{proof}

\begin{lemma}
    Let $\Dd$ be an minimal algebraic decomposition of order $k$, with leaves $V$, and let $\Tt \subseteq \powerset V$ be the underlying tree. Then the sibling relation of $\Dd$ has \mso complexity at most $f(k)$ in $(V,\Tt)$. 
\end{lemma}
For a tree $\Tt \subseteq \powerset V$, define the \emph{$\Tt$-deviation} of a subset $X \subseteq V$ to be the maximal number $k$ such that some node of $\Tt$ has at least $k$ children that contain elements from both $X$ and its complement. An equivalence relation can be viewed as a special case of a tree, where every path has length two, and the nodes at depth one are the equivalence classes. 

\begin{lemma}[Not proved]
Let $\Tt \subseteq \powerset V$ be a tree, and let $R \subseteq \powerset V$ be a relation which approximates the tree in the following sense: 
\begin{itemize}
\item $R$ selects every set that is $0$ consistent with the tree;
\item $R$ does not select any set that is 
\end{itemize}
Then the \mso complexity of $\Tt$ in $(V,\Rr)$ is 
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}[Not yet proved]
    If a decomposition is minimal, algebraic and of order $k$, then it can be defined in \mso, using the underlying hypergraph, by a formula of size $f(k)$.
\end{lemma}
